Neural Networks for Beginners. A fast implementation in Matlab, Torch, TensorFlow

This report provides an introduction to some Machine Learning tools within the most common development environments. It mainly focuses on practical problems, skipping any theoretical introduction. It is oriented to both students trying to approach Machine Learning and experts looking for new frameworks.

==> Subsections/Definitions.tex <==

\def\CpR{\textsuperscript{\sffamily\textregistered}}
\def\tt#1{\texttt{#1}}


\def\RefFig#1{Figure~\ref{#1}}
\def\RefTab#1{Table~\ref{#1}}
\def\RefEq#1{(\ref{#1})}
\def\RefEqs#1#2{(\ref{#1},\ref{#2})}
\def\RefCh#1{Chapter \ref{#1}}
\def\RefSec#1{Section~\ref{#1}}
\def\RefDef#1{Definition~\ref{#1}}
\def\RefTh#1{Theorem~\ref{#1}}
\def\RefTh#1{Conjecture~\ref{#1}}


\def\SMLtb{Statistic and Machine Learning Toolbox\textsuperscript{\tiny \texttrademark}}
\def\NNtb{Neural Network Toolbox\textsuperscript{\tiny \texttrademark}}
\def\PCtb{Parallel Computing Toolbox\textsuperscript{\tiny \texttrademark}}
\def\Cpr{\textsuperscript{\tiny \textregistered}}
\def\Ttm{\textsuperscript{\tiny \texttrademark}}
\def\MTL{\scshape Matlab}


% Matlab Code setting
\lstdefinestyle{ourMatlab}{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{gray},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Octave,                 % the language of the code
  otherkeywords={*,...},           % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{gray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=2,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{black},     % string literal style
  tabsize=2,	                   % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}

\lstdefinestyle{ourLua}{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{gray},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language={[5.0]Lua},                 % the language of the code
  otherkeywords={*,...},           % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{gray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=2,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{black},     % string literal style
  tabsize=2,	                   % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}

\lstdefinestyle{ourPython}{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{green},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=python,                 % the language of the code
  otherkeywords={*,...},           % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{gray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=2,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{black},     % string literal style
  tabsize=2,	                   % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}


\def\mcode{\lstset{style=ourMatlab}}
\def\lcode{\lstset{style=ourLua}}
\def\pcode{\lstset{style=ourPython}}



==> Subsections/shaVSdeep.tex <==
\section{Shallow vs Deep Networks}



In this section we show the difference in the behavior of a network varying its depth. Indeed, even if a 2-layer neural network is a very powerful structure, increasing the number of layer gives a complexity which allows a sensible reduction in the number of parameters.
We explain the issue illustrating some fundamental examples.



\subsection{Multidimensional XOR}



In the previous sections we saw some methods allowing us to face and to solve the XOR problem in different environments. From a theoretical point of view, a very cheap architecture able to represent the bi-dimensional XOR is given by a NN with only one hidden layer composed of two neurons with Heaviside as activation functions. In this simple case, making use of powerful architectures, we do not get significantly improvement to the performance. To appreciate how a deeper net can guarantee a better work, we pass to consider the case of the \emph{multidimensional $XOR^n$\footnote{$XOR^n:\{0;1\}^n\rightarrow\{0;1\}$ defined by $XOR^n(x_1,\ldots,x_n)=1$ iff $\displaystyle\sum_{i=1}^n x_i$ is an odd number.}}.

How is well known, each boolean formula can be rewritten in {\bf CNF} or in {\bf DNF}. This means that, given a certain n-ary boolean formula, we can automatically build up a \emph{shallow} architecture at the price of at most $2^{n-1}+1$ neurons. Each hidden neuron corresponds to an n-ary conjunction of variables, while the output neuron corresponds to a disjunction. Even if this method can be considered uniform, obviously it results too much expensive from a complexity point of view; it brings us to consider different prospective. Let us consider the following property of the $XOR^n$ function:
$$
XOR^n(x_1,\ldots,x_n)=XOR(XOR^{n-1}(x_1,\ldots,x_{n-1}),x_n).
$$
As a result, it is possible to get the n-ary $XOR^n$ iterating the application of the usual binary $XOR$ $n-1$ times, one by one, to all input. Since we need only three neurons split in two layers to compute the binary $XOR$, this time we only need $3(n-1)$ neurons, but $2(n-1)$ layers, to compute the n-ary $XOR^n$ in such a \emph{deep} network.
In order to get this last architecture, we need to separately link each input with the right layer it has to be used.
Here below, we list, as an example, the \emph{Matlab code} necessary to build up such a network for the case $n=10$. It is worth mentioning that, in this special case, we exactly know the function each neuron has to learn, so we can already set up the weights to the right values for their task. 
\mcode
\begin{lstlisting}
% DATA DEFINITION
n=10;
X = round(rand(n,2^n));
Y=(-prod((-1).^X))>0; 
P={X(1:2,:)};
for i=3:n
  P{i-1,1}=X(i,:);
end % the use of P allow us to differentiate the input types
unitsdeeps = [repmat([2,1],1,n-2),2];
ns = patternnet(unitsdeeps);
ns.numInputs=n-1;
for i=2:n-1
  ns.inputConnect(i*2-1,i)=1; 
end % to customize the input connections with the hidden layers
ns = configure(ns,P,Y);

% WEIGHTS INITIALIZATION
ns.IW{1}=[1 -1;-1 1]; % first layer weights
ns.b{1}=[-0.5; -0.5]; % first layer biases
ns.layers{1}.transferFcn='hardlim' % we set Heaviside as activation function
for i=2:2*(n-1)
  ns.layers{i}.transferFcn='hardlim'
  if mod(i,2)==0 % in even layers we have an or-neuron
    ns.LW{i,i-1}=[1 1]; % hidden layer weights
    ns.b{i}=-0.5;
  else % in even layers we have two and-neurons
    ns.LW{i, i-1}=[1; -1];
    ns.IW{i,(i+1)/2}=[-1; 1];
    ns.b{i}=[-0.5; -0.5];
  end
end
ns = train(ns,P,Y);
\end{lstlisting}
In general can be very difficult to achieve a satisfactory result training a deep network without such an \emph{ad hoc} initialization. However in this case, the provided values bring us directly to the right solution.

